The Whole is Better than the Sum: Using Aggregated Demonstrations in In-Context Learning for Sequential Recommendation

Large language models (LLMs) have shown excellent performance on various NLP tasks. To use LLMs as strong sequential recommenders, we explore the in-context learning approach to sequential recommendation. We investigate the effects of instruction format, task consistency, demonstration selection, and number of demonstrations. As increasing the number of demonstrations in ICL does not improve accuracy despite using a long prompt, we propose a novel method called LLMSRec-Syn that incorporates multiple demonstration users into one aggregated demonstration. Our experiments on three recommendation datasets show that LLMSRec-Syn outperforms state-of-the-art LLM-based sequential recommendation methods. In some cases, LLMSRec-Syn can perform on par with or even better than supervised learning methods. Our code is publicly available at https://github.com/demoleiwang/LLMSRec_Syn.

==> sections/method.tex <==
\section{Proposed Approach}
\label{sec:approach}

\subsection{Zero-Shot Method (ZS\_LLMSRec)}

To use LLM as zero-shot solver for sequential recommendation, we assume that it understands the recommendation task taking an input test user's sequence of interacted items and ranking a list of candidate items by their likelihood to be interacted next. This assumption may not hold as recommendation is usually not among the pretraining tasks. Nevertheless, we assume that LLM may have seen the past-interacted item as well as the candidate items in its pretraining. Hence, it is still able to use the item knowledge to perform reasoning over the user's preference so as to generate recommendations. 

Figure~\ref{fig:ZS-LLMRec}(a) depicts the default zero-shot prompt used for LLMRec (ZS\_LLMSRec). The prompt shows a list of watched movies as the past-interacted $x_t$, followed by the candidate movies from $D_t$.  The LLM is required to return the top-$M$ ranked candidate movies.

\subsection{One-Shot LLMSRec (OS\_LLMSRec)}

\begin{comment}
\begin{figure}[t]
     \centering
     \begin{subfigure}[b]{0.3\textwidth}
         \centering
         \includegraphics[width=\textwidth]{figures/One-Shot Prompt.png}
         \caption{One-shot LLMSRec prompting}
         \label{fig:OS-LLM_prompt}
     \end{subfigure}
     \hfill
     \begin{subfigure}[b]{0.4\textwidth}
         \centering
         \includegraphics[width=\textwidth]{figures/few-shot Prompt.png}
         \caption{Few-shot LLMSRec prompting}
         \label{fig:FS-LLM_prompt}
     \end{subfigure}
     \caption{One- and Few-Shot LLMSRec}
    \label{fig:otherLLMRec}
\end{figure}    
\end{comment}
 
\begin{figure}[t]
    \centering
    \includegraphics[width=0.5\textwidth]{figures/One-shot Prompt.png}
    \caption{One-shot LLMSRec prompting}
    \label{fig:OS-LLM_prompt}
\end{figure}

Figure~\ref{fig:OS-LLM_prompt} shows the one-shot LLM-based sequential recommendation prompting.

To select a demonstration user, we adopt the following options:
\begin{itemize}
    \item 
\end{itemize}

\subsection{Few-Shot LLMSRec (FS\_LLMSRec)}

\begin{figure*}[h]
    \centering
    \includegraphics[width=0.9\textwidth]{figures/few-shot Prompt.png}
    \caption{Few-shot LLMSRec prompting}
    \label{fig:FS-LLM_prompt}
\end{figure*}
         
Figure~\ref{fig:FS-LLM_prompt} shows the few-shot LLM-based sequential recommendation prompting.  Due to prompt length restriction, the few-shot prompt can only accommodate very few demonstration users, say 2 to 3. To accommodate more (say, > 3) demonstration users, we introduce demonstration prototype summarizing a set of demonstration users. In Figure~\ref{fig:FS-LLM_prompt}, we devise three possible few-shot prompting methods, namely:
\begin{itemize}
    \item \textit{Prompting with $k$ demonstration users}
    \item \textit{Prompting with demonstration prototype}
    \item \textit{Prompting with demonstration prototype and demonstration user}
\end{itemize}

